Diffraction-Aware Sound Localization for a Non-Line-of-Sight Source

We present a novel sound localization algorithm for a non-line-of-sight (NLOS) sound source in indoor environments. Our approach exploits the diffraction properties of sound waves as they bend around a barrier or an obstacle in the scene. We combine a ray tracing based sound propagation algorithm with a Uniform Theory of Diffraction (UTD) model, which simulate bending effects by placing a virtual sound source on a wedge in the environment. We precompute the wedges of a reconstructed mesh of an indoor scene and use them to generate diffraction acoustic rays to localize the 3D position of the source. Our method identifies the convergence region of those generated acoustic rays as the estimated source position based on a particle filter. We have evaluated our algorithm in multiple scenarios consisting of a static and dynamic NLOS sound source. In our tested cases, our approach can localize a source position with an average accuracy error, 0.7m, measured by the L2 distance between estimated and actual source locations in a 7m*7m*3m room. Furthermore, we observe 37% to 130% improvement in accuracy over a state-of-the-art localization method that does not model diffraction effects, especially when a sound source is not visible to the robot.

==> 3.tex <==
\section{Background}
\label{sec:3}

In this section, we explain a ray tracing based SSL method that our work is built upon, and motivate our work supporting the diffraction effect.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.7\columnwidth]{figures/5_computing_distance_weight.png}
	\caption{
		This figure shows an example of computing distance weights for particles $x_t^1$, $x_t^2$, and $x_t^3$ against a ray path, $R_n = [...,r_n^{k-1}, r_n^{k},...]$.
		The chosen representative distance of each particle is shown in the red color where selected perpendicular foot are $\Pi_n^1$, $\Pi_n^2$, and $\Pi_n^3$.
	}
	\vspace{-1em}
	\label{fig:computing_distance_weight}
\end{figure}

\paragraph{Reflection-aware SSL}
%As we told in Sec.~\ref{sec:2}, we already suggested 
Our work is built upon the reflection-aware
SSL~\cite{an2018reflection},
%\YOON{cite}\IK{addressed}, 
which is based on the ray-tracing technique.
%In this section, we explain the reflection-aware SSL briefly because our new
%inverse acoustic ray-tracing based SSL is developted from the prior work.
%Our prior 
It consists of two parts: performing acoustic ray tracing considering the reflection and
estimating a converging region for computing a sound source position from
those generated acoustic
rays based on
%, computed by acoustic rays using
Monte-Carlo localization (MCL).  Initially, we collect directions of the
incoming sound signals via a TDOA algorithm~\cite{valin2007robust}
%\YOON{cite}~\IK{addressed} 
and generate acoustic
rays in the opposite to those collected directions.  Although
we cannot determine whether the collected directions comes from the reflection
acoustic path or the direct path, the reflected rays are recursively generated
when any ray collides with the obstacles in the environment. Note that the
reflected acoustic ray is generated with the assumption of the specular
reflection.

This work assumes that only a single sound source exists within one frame in
an indoor environment and all sound signals are generated from that sound
source.  As a result, it indicates that we can treat
a converging region from those acoustic rays as as the estimated location of the sound source.
%should be close to the source.
%every acoustic ray travels near the
%source and
%Therefore, it is resonable to determine the converging region of rays to the estimated source position.
To identify such a converging region, we utilize MCL with randomly generated
particles as hypothetical locations of the sound source and define the
likelihood of particles.
%\YOON{Start from here...}  
The likelihood%, $P(\mathbf{o}_t| x_t^i)$, 
 of an $i$-th particle, $x_t^i$,
%is determined by the weight of each
%particle and particles are assigned to higher weights 
becomes higher as the particle gets closer to any
acoustic ray, $r_n^k$ representing a $n$-th ray with $k$-th order reflection. This is realized by the following, distance weight function:
\begin{equation}
\begin{aligned}
w_d(x_t^{i}, r_n^k) &= {f_N}(\|x_t^{i} - \pi_i^k \|\ |\ 0, \sigma_d) \cdot {F}(x_t^{i}, r_n^k),
\end{aligned}
\label{eq:distance_weight}
\end{equation}
where 
%$x_t^i$ denotes the $i$-th particle position, 
%$r_n^k$ is the $k$-th order acoustic ray, 
$\pi_i^k$ is the perpendicular foot from $x_t^i$ to $r_n^k$, $\|\cdot\|$
denotes the Euclidean distance, $f_N(\cdot)$ is the Gaussian function where the
mean is zero and the standard variance is $\sigma_d$, and $F(\cdot)$ is the
filter function returning zero to exclude irrelevant cases when the
perpendicular foot is outside of the ray segment $r_n^k$, e.g., $\pi_2^2$ in
Fig.\ref{fig:computing_distance_weight}.

%As a result, 
This approach has been demonstrated to localize a moving source even if 
the source 
generates 
%with the
intermittent sound signals and there is an obstacle blocking the
line-of-sight from the listener to the source.
%in the indoor environment.  

\paragraph{Motivations.}
While the reflection-aware SSL approach works quite well in indoor scenes with
specular materials in some parts of the scenes, we found that its accuracy
deteriorates in complex environments containing many objects.  Specifically, we
observed that in such cases with multiple objects, low-frequency effects such
as diffractions becomes an dominant issue.
%, the accuracy decreases because of the
%low-frequency effects such as diffractions.
In this work, we focus on considering the diffraction effect for robustly identifying the sound source location in scenes with many objects.
To achieve our goal, we propose a novel ray-tracing based sound source
localization algorithm using the UTD algorithm and inverse propagation signals
computed by the impulse responses of each acoustic ray.





